Multi-Layer Confidence Scoring for Detection of Out-of-Distribution Samples, Adversarial Attacks, and In-Distribution Misclassifications

The recent explosive growth in Deep Neural Networks applications raises concerns about the black-box usage of such models, with limited trasparency and trustworthiness in high-stakes domains, which have been crystallized as regulatory requirements such as the European Union Artificial Intelligence Act. While models with embedded confidence metrics have been proposed, such approaches cannot be applied to already existing models without retraining, limiting their broad application. On the other hand, post-hoc methods, which evaluate pre-trained models, focus on solving problems related to improving the confidence in the model's predictions, and detecting Out-Of-Distribution or Adversarial Attacks samples as independent applications. To tackle the limited applicability of already existing methods, we introduce Multi-Layer Analysis for Confidence Scoring (MACS), a unified post-hoc framework that analyzes intermediate activations to produce classification-maps. From the classification-maps, we derive a score applicable for confidence estimation, detecting distributional shifts and adversarial attacks, unifying the three problems in a common framework, and achieving performances that surpass the state-of-the-art approaches in our experiments with the VGG16 and ViTb16 models with a fraction of their computational overhead.

==> sections/attacks.tex <==
\section{Attack Analysis}\label{sec: attack rejection}
%
As final examination case, we choose four established attack algorithms in literature: \gls{bim} \cite{BIM}, \gls{pgd} \cite{PGD}, \gls{cw} \cite{CW} and \gls{df} \cite{DeepFool}. 
%
The analysis on attacks has been performed on \cifar{100}.
%
The attacks on both \vgg{16} and \vit{B}{16} have been computed by applying the attacks algorithm mentioned for all the images in the validation and test set.
%
In this part, we want to test whether such perturbation on the input have any effect on the corresponding \classificationmaps. 
%
To do so, we evaluate if the $\protoScore$ can differentiate between original samples and \gls{aa} by means of classical \gls{auc}.

\gls{cw} attack samples were generated using the implementation provided by the original authors \cite{CW}, and samples for the other attacks using the \codeFont{TorchAttacks} library \cite{kim2020torchattacks}.
The distance metrics used for the generation of adversarial examples are $\ell_2$ for \gls{df} and CW and $\ell_{\rm inf}$ for PGD and BIM.
%
We decide to compare the results of $\protoScore$ on attacks w.r.t. two different approaches that are well-known in literature as inference-time attack detection techniques, respectively \gls{fs}\cite{xu2017feature} and \gls{dmd}\cite{lee2018simple}. 
%
Also in this analysis we differed between \gls{dmd-a}, where the regressor has been trained on the attack that it will be tested on, and \gls{dmd-u}, where the attacks seen during training and during testing are crafted from different algorithms.
%
Moreover, we deployed the methods \gls{doc} and \gls{relu} to test whether they were generalizable to such task.
%
\begin{table}
  \centering
  \caption{Detection performance under different attacks on VGG16 and ViT-B-16.\rev{bold max}}
  \begin{tabular}{@{} 
      l      % Methods
      c c c c    % VGG16: BIM, CW, DeepFool, PGD
      c c c c    % ViT-B-16: BIM, CW, DeepFool, PGD
    @{}}
    \toprule
    \multirow{2}{*}{\textbf{Methods}}
      & \multicolumn{4}{c}{\textbf{VGG16}}
      & \multicolumn{4}{c}{\textbf{ViT-B-16}} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9}
      & BIM & CW & \gls{df} & PGD
      & BIM & CW & \gls{df} & PGD \\
    \midrule
    \gls{relu}         & 0.52 & 0.85 & 0.86 & 0.50 
                       & 0.65 & 0.84 & 0.84 & 0.54 \\
    \gls{doc}           & 0.52 & 0.94 & 0.89 & 0.43 
                       & 0.63 & 0.89 & 0.90 & 0.47 \\
    \gls{dmd-a}        & 0.79 & 0.85 & 0.94 & 0.93 
                       & 0.82 & 0.72 & 0.98 & 0.98 \\                   
    \gls{dmd-u}        & 0.70 & 0.59 & 0.81 & 0.87 
                       & 0.78 & 0.66 & 0.95 & 0.97 \\
    \gls{fs}           & 0.89 & 0.99 & 0.89 & 0.87 
                       & 0.83 & 0.99 & 0.91 & 0.78 \\
    \gls{ourframework} & 0.78 & 0.97 & 0.93 & 0.79 
                       & 0.85 & 0.97 & 0.95 & 0.85 \\
    \bottomrule
  \end{tabular}
  \label{tab: attack_metrics}
\end{table}
%
Also in this case the hyperparameters of the proposed methods \gls{dmd} and \gls{fs} where taken from the corresponding papers and in particular the configuration of filters was chosen by selecting those relative to the \cifar{10} analysis and the distance metric used to compute the score is the $\ell_1$ norm.

Tab.~\ref{tab: attack_metrics} reports the \gls{auc} values for the attack detection on both \vgg{16} and \vit{B}{16} under the attacks chosen as reference.
%
Across most settings, methods specifically tailored for attack detection \gls{fs} and \gls{dmd-a} achieve the strongest performance.
%
\gls{fs} consistently rank among the top-performing methods on both architectures, particularly under \gls{cw} and \gls{df} attacks.
%
It is worth noting that the \gls{dmd-a} configuration yields very high scores; however, these results are not directly comparable to the other methods since \gls{dmd-a} requires a regressor trained on the same attack that is used for testing. 
%
A more realistic evaluation is provided by \gls{dmd-u}, where the regressor is trained on different attacks than those used at test time. 
%
Under this more challenging and fair setting, \gls{dmd-u} performs more moderately

\gls{ourframework} achieves results comparable to the strongest baselines. By maintaining an attack-agnostic approach, it provides a robust and competitive approach.

==> sections/ood.tex <==
\section{Out-Of-Distribution}\label{sec: ood}

A key requirement for reliable models is robustness to \gls{ood} data. To examine this, we test \gls{ourframework} on corrupted samples from \cifar{100C}, leveraging the \protoclasses' score ($\protoScore$) as the detection metric.

\gls{ourframework} is compared with \gls{sota} methods for \gls{ood} detection \gls{msp}\cite{hendrycks2017baseline}, \gls{doc}\cite{granese2021doctor}, \gls{relu}\cite{dadalto2023data} and \gls{dmd}\cite{lee2018simple}.
%
As quantitative result, we evaluate the performances of detection of corrupted samples in terms of \gls{auc}.

Figure \ref{fig: corruption} shows the scores distributions of each method for \gls{id} samples, taken from \cifar{100}'s $\testSet$, in comparison to \cifar{100C} according to the corruption levels.
%
One can observe that \gls{msp} is over-confident for \gls{id} samples, meaning they are attributed a high score value.
%
Even though the confidence decreases for corrupted samples according to the corruption intensity, the shift in the distributions overlap is subtle, indicating that the model's confidence is not sufficient for corruption detection and corroborating with the results from \cite{liang2017enhancing}.
%
On the other hand, the $\protoScore$'s distribution shifts more quickly as the corruption intensity increases. 
%
\gls{dmd} extract information from multiple layers, as \gls{ourframework}, and combine it by training a linear regressor to classify between original samples and corrupted one. 
%
Even if the \gls{dmd} detector transforms the detection in a binary classification task we can state that \gls{ourframework} reaches comparable results in terms of \gls{auc} both on the \vgg{16} and the \vit{B}{16}.  

\begin{figure*}
    \centering
    \begin{subfigure}[b]{\textwidth}
    	\centering
    	\includegraphics[width=\linewidth]{figures/CIFAR100_vgg16/in_out_distribution}
    	\caption{\vgg{16}.}
    	\label{fig: ood vgg cifar100}	
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
    	\centering
    	\includegraphics[width=\linewidth]{figures/CIFAR100_ViT/in_out_distribution}
    	\caption{\vit{B}{16}.}
    	\label{fig: ood vit cifar100}	
    \end{subfigure}
    \caption{Scores distribution for \cifar{100C}. \gls{id} samples correspond to \cifar{100}'s \testSet and are assigned with label $1$, $cX$ correspond to \cifar{100C} for each corruption intensity, and are assigned with label $0$. The \gls{auc} values (right-most plot) show that the proposed score $\protoScore$ outperforms the model's confidence on \gls{ood} identification.}
    \label{fig: corruption}
\end{figure*}

To further assess the utility of \classificationmaps representations, we analyze their effectiveness in an \gls{ood} detection setting.
%
Specifically, we consider \vgg{16} and \vit{B}{16} models trained on \cifar{100}, and evaluate their behavior on \SVHN and \places, which serve as reference \gls{ood} datasets \cite{yang2022fsood}.
%
The discriminative power of the $\protoScore$ in separating \gls{id} from \gls{ood} samples is quantified also in this case by the \gls{auc} metric. 
%
The results are summarized in Tab.~\ref{tab: ood metrics}, where we compare \gls{ourframework} against established \gls{sota} methods mentioned before.

For comparison, we also evaluate the \gls{dmd} approach in two settings: in the aware case (\gls{dmd-a}), the regressor is trained and tested on the same \gls{ood} distribution, whereas in the more realistic unaware case (\gls{dmd-u}), training and test distributions differ, reflecting conditions where the nature of the shift cannot be anticipated in advance.
%
The results for \vgg{16} reveal that, on the \places dataset, \gls{dmd} achieves the strongest performance among the compared methods in both the aware and unaware settings. 
%
However, when evaluated on \SVHN, performance degrades substantially for both \gls{dmd-a} and \gls{dmd-u}, with the latter being comparable to the results obtained by the model confidence baseline and the proposed $\protoScore$.
%
In contrast, experiments with \vit{B}{16} yield more promising results: the $\protoScore$ achieves near-perfect detection performance on both \gls{ood} datasets without requiring any additional retraining, in contrast to the overhead associated with \gls{dmd}.

\begin{table}
  \centering
  \caption{Detection performance in terms of \gls{auc} of \gls{ood} dataset given \cifar{100} as \gls{id} dataset on VGG16 and ViT-B-16.}
  \begin{tabular}{@{} 
      l      % Methods
      c c    % VGG16: Places, SVHN
      c c    % ViT-B-16: Places, SVHN
    @{}}
    \toprule
    \multirow{2}{*}{\textbf{Methods}}
      & \multicolumn{2}{c}{\textbf{VGG16}}
      & \multicolumn{2}{c}{\textbf{ViT-B-16}} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5}
      & \places & \SVHN 
      & \places & \SVHN  \\
    \midrule
    \gls{msp}\cite{hendrycks2017baseline}   & 0.84 & 0.82  
                                            & 0.84 & 0.90  \\
    \gls{doc}\cite{granese2021doctor}       & 0.84 & 0.82  
                                            & 0.85 & 0.91  \\
    \gls{relu}\cite{dadalto2023data}        & 0.74 & 0.64  
                                            & 0.67 & 0.67  \\
    \gls{dmd-a}\cite{lee2018simple}         & 0.99 & 0.87  
                                            & 0.99 & 0.98  \\
    \gls{dmd-u}                             & 0.99 & 0.80  
                                            & 0.03 & 0.50  \\
    \gls{ourframework}                      & 0.84 & 0.80  
                                            & 0.99 & 0.99  \\
    \bottomrule
  \end{tabular}
  \label{tab: ood metrics}
\end{table}
 
